ADEPT: A Dataset for Evaluating Prosody Transfer

Text-to-speech is now able to achieve near-human naturalness and research focus has shifted to increasing expressivity. One popular method is to transfer the prosody from a reference speech sample. There have been considerable advances in using prosody transfer to generate more expressive speech, but the field lacks a clear definition of what successful prosody transfer means and a method for measuring it. We introduce a dataset of prosodically-varied reference natural speech samples for evaluating prosody transfer. The samples include global variations reflecting emotion and interpersonal attitude, and local variations reflecting topical emphasis, propositional attitude, syntactic phrasing and marked tonicity. The corpus only includes prosodic variations that listeners are able to distinguish with reasonable accuracy, and we report these figures as a benchmark against which text-to-speech prosody transfer can be compared. We conclude the paper with a demonstration of our proposed evaluation methodology, using the corpus to evaluate two text-to-speech models that perform prosody transfer.

==> LaTeX/IEEEtran/tools/README <==

January 11, 2007


The IEEEtrantools.sty package provides several commands from the
IEEEtran.cls file so that they can be used under other LaTeX classes. The
user guide provided here covers only the differences in the use of the
commands from those provided by IEEEtran.cls. For complete documentation
on these commands, see the relevant sections in the IEEEtran_HOWTO manual
of the IEEEtran LaTeX class.

The IEEEtrantools.sty package provides the following IEEEtran.cls commands:

 1. \IEEEPARstart which produces large initial "drop cap" letters.
 2. the \bstctlcite command for the control entry types of IEEEtran.bst
    V1.00 and later
 3. the IEEE itemize, enumerate and description list environments
 4. the complete IEEEeqnarray family for producing multiline equations
    as well as matrices and tables, including the IEEEeqnarray support
    commands.

IEEEtrantools.sty should not be used with IEEEtran.cls.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtrantools support page at my website:

http://www.michaelshell.org/tex/ieeetran/tools/


Enjoy!

Michael Shell
http://www.michaelshell.org/


*******
1/2007 V1.2 (V1.7 of IEEEtran.cls) changes:

 1. Several commands and enviroments have depreciated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow use of the
    obsolete forms, but with an warning message to the console during
    compilation:
    \IEEEPARstart
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
 
 2. These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. \normalsizebaselineskip no longer provided. 

 4. New \IEEEPARstart controls:
    \IEEEPARstartHEIGHTTEXT, \IEEEPARstartFONTSTYLE, \IEEEPARstartCAPSTYLE,
    \IEEEPARstartWORDFONTSTYLE, \IEEEPARstartWORDCAPSTYLE,
    \IEEEPARstartHOFFSET, \IEEEPARstartITLCORRECT
    and the (output) length \IEEEPARstartletwidth.

 5. Provide for an optional argument to \bstctlcite to provide a way to
    specify a different aux file. Define \bstctlcite even if it has already
    been defined.

********************************** Files **********************************

README                - This file.

IEEEtrantools.sty     - The LaTeX package file.

IEEEtrantools_doc.txt - The user manual - supplementary to the 
                        IEEEtran_HOWTO manual.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtrantools.sty, IEEEtrantools_doc.txt
***************************************************************************



==> horizontal_figure.tex <==
\begin{figure*}[h]
\centering
    \begin{multicols}{4}
    \hspace*{5.5em}Female or LJ
    \vfill
    \hspace*{2em}Male or Proprietary\vfill
    Female or LJ
    \vfill
    \hspace*{-3.5em}
    Male or Proprietary
    \end{multicols}
    \vspace{-1.1\baselineskip}
    \begin{subfigure}[b]{\columnwidth}
    \includegraphics[width=0.49\columnwidth]{Images/emotion_00.pdf}\hfil
    \includegraphics[width=0.49\columnwidth]{Images/emotion_01.pdf}\hfil
    \vspace{-0.5\baselineskip}
    \caption{Emotion}
    \end{subfigure}
    \begin{subfigure}[b]{\columnwidth}
    \includegraphics[width=0.49\columnwidth]{Images/int_att_00.pdf}\hfil
    \includegraphics[width=0.49\columnwidth]{Images/int_att_01.pdf}
    \vspace{-0.5\baselineskip}
    \caption{Interpersonal attitude}
    \par\medskip
    \end{subfigure}
    \begin{subfigure}[b]{\columnwidth}
    \includegraphics[width=0.49\columnwidth]{Images/emphasis_00.pdf}\hfil
    \includegraphics[width=0.49\columnwidth]{Images/emphasis_01.pdf}\hfil
    \vspace{-0.5\baselineskip}
    \caption{Topical emphasis}
    \end{subfigure}
    \begin{subfigure}[b]{\columnwidth}
    \includegraphics[width=0.49\columnwidth]{Images/prop_att_00.pdf}\hfil
    \includegraphics[width=0.49\columnwidth]{Images/prop_att_01.pdf}
    \vspace{-0.5\baselineskip}
    \caption{Propositional attitude}
    \par\medskip
    \end{subfigure}
    \begin{subfigure}[b]{\columnwidth}
    \includegraphics[width=0.49\columnwidth]{Images/syn_phrase_00.pdf}\hfil
    \includegraphics[width=0.49\columnwidth]{Images/syn_phrase_01.pdf}\hfil
    \vspace{-0.5\baselineskip}
    \caption{Syntactic phrasing}
    \end{subfigure}
    \begin{subfigure}[b]{\columnwidth}
    \includegraphics[width=0.49\columnwidth]{Images/mark_ton_00.pdf}\hfil
    \includegraphics[width=0.49\columnwidth]{Images/mark_ton_01.pdf}
    \vspace{-0.5\baselineskip}
    \caption{Marked tonicity}
    \end{subfigure}
\vspace{-0.5\baselineskip}
\caption{Recognition accuracy of each category for the female and male speaker samples from the natural recordings, and the LJSpeech and proprietary speakers for the T-Ctrl and Tacotron-Ref models. Chance performance is indicated by a horizontal dashed line. Error bars indicate one standard deviation (estimated by scaling the per speaker standard error).}
\label{fig:final_results}
\end{figure*}

==> vertical_figure.tex <==
\begin{figure}
    \centering
    \begin{multicols}{2}
    \hspace*{3em}Female or LJ
    \vfill
    Male or Proprietary
    \end{multicols}
    \begin{subfigure}[b]{\columnwidth}
        \centering
        \includegraphics[width=0.5\columnwidth]{Images/emotion_00.pdf}%
        \hfill
        \includegraphics[width=0.5\columnwidth]{Images/emotion_01.pdf}
        \vspace{-1.7\baselineskip}
        \caption{Emotion}
    \end{subfigure}     
    \label{fig:emotion}
     
    \begin{subfigure}[b]{\columnwidth}
        \centering
        \includegraphics[width=0.5\columnwidth]{Images/int_att_00.pdf}%
        \hfill
        \includegraphics[width=0.5\columnwidth]{Images/int_att_01.pdf}
        \vspace{-1.7\baselineskip}
        \caption{Interpersonal Attitude}  
    \end{subfigure} 
    \begin{subfigure}[b]{\columnwidth}
        \centering
        \includegraphics[width=0.5\columnwidth]{Images/emphasis_00.pdf}%
        \hfill
        \centering
        \includegraphics[width=0.5\columnwidth]{Images/emphasis_01.pdf}
        \vspace{-1.7\baselineskip}
        \caption{Topical Emphasis}
    \end{subfigure}     
    \label{fig:emphasis}
    
    \begin{subfigure}[b]{\columnwidth}
        \centering
        \includegraphics[width=0.5\columnwidth]{Images/prop_att_00.pdf}%
        \hfill
        \includegraphics[width=0.5\columnwidth]{Images/prop_att_01.pdf}
        \vspace{-1.7\baselineskip}
        \caption{Propositional Attitude}
    \end{subfigure}     
    \label{fig:prop_att}

    \begin{subfigure}[b]{\columnwidth}
        \centering
        \includegraphics[width=0.5\columnwidth]{Images/syn_phrase_00.pdf}%
        \hfill
        \includegraphics[width=0.5\columnwidth]{Images/syn_phrase_01.pdf}
        \vspace{-1.7\baselineskip}
        \caption{Syntactic Phrasing}
    \end{subfigure}     
    \label{fig:syn_phrase}
     
    \begin{subfigure}[b]{\columnwidth}
        \centering
        \includegraphics[width=0.5\columnwidth]{Images/mark_ton_00.pdf}%
        \hfill
        \includegraphics[width=0.5\columnwidth]{Images/mark_ton_01.pdf}
        \vspace{-1.7\baselineskip}
        \caption{Marked Tonicity}
    \end{subfigure}     
    \label{fig:mark_ton}    
    \label{fig:int_att}
    \vspace{-1\baselineskip}
    \caption{Recognition accuracy of each category for the female and male speaker samples from the natural recordings, and the LJSpeech and proprietary speakers for the TCESS and Tacotron-Ref models. Chance performance is indicated by a horizontal dashed line. Error bars indicate one standard deviation (estimated by scaling the per speaker standard error).}
    \label{fig:final_results}
\end{figure}
